Beam Profiling and Beamforming Modeling for mmWave NextG Networks

This paper presents an experimental study on mmWave beam profiling on a mmWave testbed, and develops a machine learning model for beamforming based on the experiment data. The datasets we have obtained from the beam profiling and the machine learning model for beamforming are valuable for a broad set of network design problems, such as network topology optimization, user equipment association, power allocation, and beam scheduling, in complex and dynamic mmWave networks. We have used two commercial-grade mmWave testbeds with operational frequencies on the 27 Ghz and 71 GHz, respectively, for beam profiling. The obtained datasets were used to train the machine learning model to estimate the received downlink signal power, and data rate at the receivers (user equipment with different geographical locations in the range of a transmitter (base station). The results have shown high prediction accuracy with low mean square error (loss), indicating the model's ability to estimate the received signal power or data rate at each individual receiver covered by a beam. The dataset and the machine learning-based beamforming model can assist researchers in optimizing various network design problems for mmWave networks.

==> sections/archive.tex <==

 %Based on Table \ref{table_NN_Layers}, the 5-layer model has the best performance, while adding one more layer (6-layer model) results in a decreased performance.


%Table \ref{table_NN_Layers}  shows the R2 values of different NN architectures with varying numbers of hidden% layers and neurons for two distinct datasets. 
%This analysis can aid in identifying the optimal neural network configuration for a given problem. Notably, the five-layer NN architecture outperformed the other NN architectures, suggesting that a deeper network can learn more intricate representations of the input data, thereby enhancing its accuracy in predicting the outcome of the task. On the other hand, too many layers may hurt the performance, e.g., due to overfitting and various other issues. Based on, Table \ref{table_NN_Layers}, the 5-layer model has the best performance, while adding one more layer (6-layer model) results in a decreased performance.

%the NN improved its ability to capture the non-linear relationships between the input and output variables.

%In order to explore the optimal number of neurons and layers which achieve that achieves the best performance in a prediction task, we conducted a comparison of the performance of various NN architectures, including the NN-5layer model.  The findings presented in the table indicate that augmenting the number of layers in the NN enhanced its capacity to capture the non-linear associations between the input and output variables.




%\hl{please check all table and figure cross reference, to make sure they are right.here I corrected the Table reference from table2 to tableNNLayers.}
%%Table \ref{table2} 



%\hl{need to clarify the InterDigtal dataset output is RSRP and the unit is dbm. the MSE result is computed based on those dbm values. similar for NI data results. }

%The performance of the MSE as a loss function was analyzed for two datasets, InterDigital and NI-generated. The results are depicted in  \figurename{\ref{fig:Loss}}, where the blue line represents the InterDigital dataset and the yellow line represents the NI-obtained dataset.The InterDigital dataset had an initial loss value of 0.78, which rapidly decreased to 0.25 after 14 epochs. Subsequently, the loss value slightly decreased further and reached its minimum value after 200 epochs. On the other hand, the NI-obtained dataset also exhibited a similar trend. Its initial loss value was 0.85, which decreased to 0.3 after 18 epochs and reached its minimum value at the end of the training process. Overall, the analysis shows that both datasets exhibited a significant reduction in the loss function value over the training process. The InterDigital dataset achieved a slightly better performance in terms of the final loss value.

%To ensure the effectiveness of the selected features, number of neurons, and layers of the designed NN model, we compared NN-5layer model with ifferent NN architectures in the context of a prediction task, showing deeper networks' benefits for achieving better performance. The ability to capture the non-linear relationships between the input and output variables was improved by increasing the number of layers in the NN. In table \ref{table2}, the R2 values of various neural network architectures with different numbers of hidden layers and neurons are compared for two different datasets. This analysis can assist in identifying the best neural network configuration for a given issue. Consequently, it was found that the five-layer NN architecture performed better than other NN architectures. Specifically, this suggests that a deeper network can learn more intricate representations of the input data, which will improve its accuracy in predicting how the task will turn out.

%\subsubsection{Comparison between NN-5layers model and other NN structures}


%In addition, we compared the prediction performance of various classical ML models for selecting the optimal ML algorithm for a given dataset. For this purpose, factors such as the complexity and non-linearity of the underlying relationships must be considered. Hence, we evaluate our model (NN-5layers) with five commonly used regression algorithms: Linear regressions, CatBoostRegressor, RandomForestRegressor, GradientBoostingRegressor. Linear regression is a statistical method that models the linear relationship between a dependent variable and one or more independent variables. The CatBoostRegressor and RandomForestRegressor are ensemble methods based on decision trees that utilize multiple decision tree outputs to enhance prediction accuracy. These algorithms are suitable for handling non-linear relationships between features and the target variable. The GradientBoostingRegressor, another ensemble method based on decision trees, employs gradient boosting to improve the performance of individual trees. This algorithm typically achieves better accuracy than random forests, although it may be slower to train and more challenging to fine-tune. the last one is the NN models with three fully connected hidden layers (NN-3layers). 



%developed two different neural network models, the first model is composed of three fully connected hidden layers, while the other neural network model consists of five fully connected hidden layers. The results of this study, which


%Based on the evaluation metrics, the NN-5layers model shows a relatively low MSE during the training phases for both InterDigital and NI datasets, as depicted in \figurename{\ref{fig:Loss}}. The average MSE value for training the model with the Interdigital and NI dataset was about 0.16 and 0.17, respectively. The InterDigital dataset had an initial loss value of 0.78, which rapidly decreased to 0.25 after 14 epochs. Subsequently, the loss value slightly decreased further and reached its minimum value after 200 epochs. On the other hand, the NI-obtained dataset also exhibited a similar trend. Its initial loss value was 0.85, which decreased to 0.3 after 18 epochs and reached its minimum value at the end of the training process. Overall, the analysis shows that both datasets exhibited a significant reduction in the loss function value over the training process. The InterDigital dataset achieved a slightly better performance in terms of the final loss value.



%\begin{subfigure}[b]{0.5\textwidth}
        %\centerline{\includegraphics[scale=0.45]{sections/Difference-3Layer.png}}
     %   \caption{Ground truth VS Predicted value for ~\cite{kazemi2022channel}}
     %   \label{fig:Comparison-onothermodel}
    % \end{subfigure}


%Based on the experimentation with different regression models, the Neural Network model architecture is deemed to be the most suitable fit for the dataset. The Neural Network model comprises five densely connected layers, employing Tanh and ReLU activation functions for the input and hidden layers. The input includes three features, namely $\alpha$, $\beta$, and $d$, which serve as the basis for the network's computation. The first hidden layer of the network consists of 32 neurons, with the number of neurons gradually decreasing towards the output layer. The output layer contains a single neuron that represents the predicted communication quality strength of the user equipment (UE). The evaluation of these models in terms of the aforementioned metrics is demonstrated in Section VI-C. 



%In Section V of the paper, it was explained that the MSE function was used to compare the different ML models used in the study. \figurename{\ref{fig:MSE-Inter}} illustrates the comparison of the InterDigital dataset, where it can be observed that our proposed model achieves the lowest MSE value of 0.16, followed by the Cat Boost Regressor with the second-lowest value, and the Neural Network model with three layers and Gradient Boosting Regressor achieving relatively higher MSE values. However, Linear Regression stands out as the worst-performing model, obtaining the highest value of the loss function with 0.35. \figurename{\ref{fig:MSE-NI}} displays the same metric for the NI dataset, where it can be observed that our proposed model also obtains the lowest MSE value of 0.17, then the Neural Network model with three layers has the second-lowest value of 0.23. In contrast, Cat Boost Regressor and Random Forest Regressor achieved MSE values of 0.25 and 0.27, respectively. As with the InterDigital dataset, Linear Regression performs the worst on the NI dataset as well. Overall, the results from both datasets indicate that our proposed model and the Neural Network model with three layers perform the best among the compared ML models, while Linear Regression performs the worst.

%The obtained R2 values for InterDigital and NI-obtained datasets demonstrated a significant improvement in performance. The R2 value for InterDigital dataset was 0.98, while for NI-obtained dataset, it was 0.96. \figurename{\ref{fig:ML-comparison}} illustrates the R2 values obtained from different ML approaches applied to the two datasets. For InterDigital dataset, \figurename{\ref{fig:ML-Inter}}, the Cat Boost Regressor obtained the second highest R2 value of 0.96, followed by the NN model with 3 layers and Gradient Boosting Regressor, both of which reached an R2 value of 0.94 and shared the third position. For NI-obtained dataset (\figurename{\ref{fig:ML-NI}}), the NN model with 3 layers achieved the second highest R2 value of 0.93 after our model with five layers of Neural network. At the same time, the Cat Boost Regressor obtained the third position with an R2 value of 0.91. The other ML models, including Random Forest Regressor, Gradient Boosting Regressor, and Linear Regression, received lower R2 values. Overall, the analysis demonstrated that the applied ML approaches shows significant improvement in predicting the performance of the datasets. Some approaches, such as the NN model with five layers and Cat Boost Regressor, shows superior performance compared to other approaches.

%This indicates that the neural network model can make accurate predictions for both datasets, and its proposed design factor demonstrated its effectiveness. The model's ability to predict communication quality strength reliably allows for determining the best beam selection and node association estimation in real time. Nonetheless, the model can be enhanced by expanding the size of the datasets and optimizing the network architecture.




%\begin{figure}[ht]
%\centerline{\includegraphics[scale=0.50]{sections/Fig9.png}}
%\caption{NN Loss function for InterDigital-based dataset}
%\label{fig:fig9}
%\end{figure}


%\begin{figure}[ht]
%\centerline{\includegraphics[scale=0.50]{sections/Fig10.png}}
%\caption{NN Loss function for NI-based dataset}
%\label{fig:fig10}
%\end{figure}

